FastCPH: Efficient Survival Analysis for Neural Networks

The Cox proportional hazards model is a canonical method in survival analysis for prediction of the life expectancy of a patient given clinical or genetic covariates -- it is a linear model in its original form. In recent years, several methods have been proposed to generalize the Cox model to neural networks, but none of these are both numerically correct and computationally efficient. We propose FastCPH, a new method that runs in linear time and supports both the standard Breslow and Efron methods for tied events. We also demonstrate the performance of FastCPH combined with LassoNet, a neural network that provides interpretability through feature sparsity, on survival datasets. The final procedure is efficient, selects useful covariates and outperforms existing CoxPH approaches.

==> algorithms/algorithm_breslow.tex <==
\begin{algorithm}
\caption{\textsc{FastCPH - Breslow Method }}\label{alg:breslow}
\textbf{Input:} Neural network output $\textbf{H}=g(\textbf{x})$, duration $\textbf{T}$, events $\textbf{E}$\\
\textbf{Output:} Negative CoxPH partial log likelihood using Breslow Method\\
\textbf{Assumption:} \textbf{H} and \textbf{E} sorted in descending order w.r.t \textbf{T}.
\begin{algorithmic}
\State $\textbf{J} \gets$ nonzero indices of $\mathbf{E}$ 
\State $S_1 \gets$ sum of \textbf{H} at \textbf{J}
\Comment{Eq \ref{eq:breslow_1}}
\State $\textbf{J'} \gets$ unique events in \textbf{J}
\State $d_j' \gets$ event counts for each unique $j' \in \textbf{J'}$ 
\State $S_2 \gets d_j' \cdot \texttt{logcumsumexp}(\textbf{H}) $ at $j' \in \textbf{J'}$
\Comment{Eq \ref{eq:breslow_2}}\\
\Return $S_2 - S_1$
\Comment{Eq \ref{eq:breslow_0}}
\end{algorithmic}
\end{algorithm}





==> algorithms/algorithm_no_ties.tex <==
\begin{algorithm}
\caption{\textsc{FastCPH - No ties}}\label{alg:no_ties}
\textbf{Input:} Neural network output $\textbf{H}=g(\textbf{x})$, duration $\textbf{T}$, events $\textbf{E}$\\
\textbf{Output:} Negative CoxPH partial log likelihood \\
\textbf{Assumption:} No ties in \textbf{T}. \textbf{H} and \textbf{E} sorted in descending order w.r.t \textbf{T}.
\begin{algorithmic}
\State $\textbf{L} \gets$ $\texttt{logcumsumexp(}\textbf{H}\texttt{)}-$ \textbf{H}
\Comment{Eq \ref{eq:no_ties_1}}\\
\Return $\textbf{L}^{T}\cdot $ \textbf{E}
\end{algorithmic}
\end{algorithm}

==> figures/include_hnscc_curve.tex <==
\begin{figure*}[ht]
  \centering
  \vspace{5mm}
    \includegraphics[width=100mm]{figures/HNSCC_curve.png}
  
  \caption{The training curve for \textit{FastCPH-LassoNet} on HNSCC dataset. This is one run with setting of the best model for HNSCC dataset in Table \ref{hyperparam}. The red vertical lines represent the mean value of the best model of 5 random trails using the same setting. The best model is selected by validation accuracy among different $\lambda$. The red dotted lines indicate 95\% CI.  Similar to Fig \ref{fig:experiment_1}, the first figure is the number of selected features versus the test C-index. The second figure represents the change in test score when $\lambda$ increases during training. The third figure is the number of features selected when $\lambda$ increases during training. }
  \label{fig:hnscc_curve}
\vspace{5mm}
\end{figure*}

==> figures/include_loss_comparison.tex <==
\begin{figure*}
  \centering
  \vspace{5mm}
    \includegraphics*[width=100mm]{figures/loss_comparison.png}
  \label{fig:loss_comparison}
  \caption{Comparison of \textit{FastCPH} with the Breslow method and PyCox Loss. This figure is the validation loss of two \textit{LassoNet} backbones trained on \textit{LassoNet} and Pycox loss. As we can see in the figure, while two loss obtain global minimum at similar $\lambda$, the magnitude of \textit{FastCPH} is smaller than of PyCox, which does not support ties.}
\vspace{5mm}
\end{figure*}
